Adaptive Human-Robot Collaborative Missions using Hybrid Task Planning

Producing robust task plans in human-robot collaborative missions is a critical activity in order to increase the likelihood of these missions completing successfully. Despite the broad research body in the area, which considers different classes of constraints and uncertainties, its applicability is confined to relatively simple problems that can be comfortably addressed by the underpinning mathematically-based or heuristic-driven solver engines. In this paper, we introduce a hybrid approach that effectively solves the task planning problem by decomposing it into two intertwined parts, starting with the identification of a feasible plan and followed by its uncertainty augmentation and verification yielding a set of Pareto optimal plans. To enhance its robustness, adaptation tactics are devised for the evolving system requirements and agents' capabilities. We demonstrate our approach through an industrial case study involving workers and robots undertaking activities within a vineyard, showcasing the benefits of our hybrid approach both in the generation of feasible solutions and scalability compared to native planners.

==> PDDL/json.tex <==
{
    "_comment": "Locations",
    "locations": [
      {
        "id": "l1",
        "description": "Initial location.",
        "coordinates": { "x": 1, "y": 1 }
      },
      {
        "id": "l2",
        "description": "Location to the right of location.",
        "coordinates": { "x": 1, "y": 2 }
      },
      {
        "id": "l3",
        "coordinates": { "x": 1, "y": 3 }
      },
      {
        "id": "l4",
        "coordinates": { "x": 2, "y": 1 }
      },
      {
        "id": "l5",
        "coordinates": { "x": 2, "y": 2 }
      },
      {
        "id": "l6",
        "coordinates": { "x": 2, "y": 3 }
      },
      {
        "id": "l7",
        "coordinates": { "x": 3, "y": 1 }
      },
      {
        "id": "l8",
        "coordinates": { "x": 3, "y": 2 }
      },
      {
        "id": "l9",
        "coordinates": { "x": 3, "y": 3 }
      }
    ],




    "_comment": "Paths bidirectional",
    "paths": [
    {
      "start_location": "l1",
      "end_location": "l2",
      "path_description": "Path from l1 to l2",
      "distance": 1
    },
    {
      "start_location": "l1",
      "end_location": "l4",
      "path_description": "Path from l1 to l4",
      "distance": 1
    },
    {
      "start_location": "l2",
      "end_location": "l3",
      "path_description": "Path from l2 to l3",
      "distance": 1
    },
    {
      "start_location": "l2",
      "end_location": "l5",
      "path_description": "Path from l2 to l5",
      "distance": 1
    },
    {
      "start_location": "l3",
      "end_location": "l6",
      "path_description": "Path from l3 to l6",
      "distance": 1
    },
    {
      "start_location": "l4",
      "end_location": "l5",
      "path_description": "Path from l4 to l5",
      "distance": 1
    },
    {
      "start_location": "l4",
      "end_location": "l7",
      "path_description": "Path from l4 to l7",
      "distance": 1
    },
    {
      "start_location": "l5",
      "end_location": "l6",
      "path_description": "Path from l5 to l6",
      "distance": 1
    },
    {
      "start_location": "l5",
      "end_location": "l8",
      "path_description": "Path from l5 to l8",
      "distance": 1
    },
    {
      "start_location": "l6",
      "end_location": "l9",
      "path_description": "Path from l6 to l9",
      "distance": 1
    },
    {
      "start_location": "l7",
      "end_location": "l8",
      "path_description": "Path from l7 to l8",
      "distance": 1
    },
    {
      "start_location": "l8",
      "end_location": "l9",
      "path_description": "Path from l8 to l9",
      "distance": 1
    }
  ],

  
  "_comment": "Tasks",
  "tasks": [
    {
      "id": "t1",
      "description": "Task t1",
      "duration": 1,
      "instances": [
        {
          "id": "t1l4", "location": "l4"
        },
        {
          "id": "t1l6a", "location": "l6"
        },
        {
          "id": "t1l6b", "location": "l6"
        },
        {
          "id": "t1l7", "location": "l7"
        }
      ]
    },
    {
      "id": "t2",
      "description": "Task t2",
      "duration": 1,
      "instances": [
        {
          "id": "t2l5",
          "location": "l5"
        },
        {
          "id": "t2l8a", "location": "l8"
        },
        {
          "id": "t2l8b", "location": "l8"
        }
      ]
    },
    {
      "id": "t3",
      "description": "Task t3",
      "duration": 1,
      "instances": [
        {
          "id": "t3l4", "location": "l4"
        },
        {
          "id": "t3l7", "location": "l7"
        },
        {
          "id": "t3l9", "location": "l9"
        }
      ]
    }
  ],





    "_comment": "Agents",
    "agents": [
      {
        "id": "worker1",
        "type": "worker",
        "tasks": [
          {
            "type": "t1",
            "probability_of_success": 1.00,
            "cost": 3,
            "number_of_retries": 5
          },
          {
            "type": "t3",
            "probability_of_success": 0.99,
            "cost": 5,
            "number_of_retries": 5
          }
        ]
      },
      {
        "id": "worker2",
        "type": "worker",
        "tasks": [
          {
            "type": "t1",
            "probability_of_success": 1.00,
            "cost": 3,
            "number_of_retries": 5
          },
          {
            "type": "t3",
            "probability_of_success": 0.99,
            "cost": 5,
            "number_of_retries": 5
          }
        ]
      },
      {
        "id": "r1",
        "type": "robot",
        "tasks": [
          {
            "type": "t2",
            "probability_of_success": 0.99,
            "cost": 1,
            "number_of_retries": 10
          },
          {
            "type": "t3",
            "probability_of_success": 0.97,
            "cost": 1,
            "number_of_retries": 10
          }
        ]
      }
    ]
}


==> Tables/table-RQ1-inSec-NOTUSED.tex <==
\begin{table*}[]
\caption{Hybrid approach compared to a full-MDP model}
\vspace{-4mm}
%\url{https://docs.google.com/spreadsheets/d/1Iwyae02-TFwfa7iDuavsNNzRzTQacH21bkYkkwidn8A/edit?gid=1195719558#gid=1195719558}}
\label{table:fullMDP}
%\centering
\sffamily
\begin{scriptsize}
\begin{center}
\resizebox{\textwidth}{!}{ % Resizes the table to fit the text width
\begin{tabular}{p{0.5cm}|p{0.1cm}p{0.1cm}p{0.4cm}p{1.85cm}|p{1.0cm}p{1.2cm}p{1.6cm}p{0.4cm}|p{0.8cm}p{0.80cm}llp{1.5cm}}
\toprule%{2-12}
%\cline{2-12}

 \multicolumn{5}{c|}{\textbf{Planning problem}} 
 
 & \multicolumn{4}{c|}{\textbf{Full MDP verification approach}} 
 
 & \multicolumn{5}{c}{\textbf{Hybrid approach}}
 
 \\
\cline{2-11}
%\midrule
\hline

ID & $|T|$ & $|L|$ & retries & agents

& \multicolumn{1}{l}{\#states} & \multicolumn{1}{l}{\#trans} & \begin{tabular}[c]{@{}l@{}}PMC\\execution\\mean time\\ (SD) [s]\end{tabular} & $|PS|$ &  \# states* & \# trans*
& \begin{tabular}[c]{@{}l@{}}Numerical\\planner\\mean time\\ (SD) [s] \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Verif.\\\& search\\mean time\\ (SD) [m]\end{tabular} 
&  \begin{tabular}[c]{@{}l@{}} $|PS|$ \\ mean (SD) \end{tabular} \\
%\midrule
\hline



% 0.2976666666666667 0.024590905710814327
% 0.33266666666666667 0.02490441497119479
% 0.33066666666666666 0.024625937172201094
% 2.0283333333333333 0.08238192525788293

$\mathcal{M}_1$ & 3 & 9 & 1 & 1 human, 1 robot & 35,081 & 172,714 & 196.69 (85.38)  & 3  & 14 & 17 & 0.29 (0.02) & 1.76 (0.92)  & 1 (0.00) \\ %p = 0.9999999999333901, 0.999946000729
%problem3 in data

\textbf{$\mathcal{M}_2$} & 2 & 6 & 3 & 1 human, 1 robot & 134,581 & 541,767 & 128.53 (53.93) & 3  &  36 & 48 & 0.33 (0.02) & 1.73 (0.03) & 4 (0.00)  \\ % Result: [(0.9999729999730006, 4.063123524275327)]
%problem1 in data

$\mathcal{M}_3$ & 3 & 9 & CS & 2 human, 2 robot & 270,100,547 & 1,351,524,022 & Timeout  & - & 398 & 553 & 0.33 (0.02) & 14.73 (2.30) & 47.80 (7.87)  \\ %0.99999999793485
%problem4 in data
$\mathcal{M}_4$ & 10 & 9 & CS & 2 human, 2 robot & OOM & OOM &  - & - & 1,825,976 & 3,822,145 & 
2.02 (0.08) & 2.13 (0.17) & 39.93 (3.17) \\ %0.9999999963720143
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-1mm}
\text{*} from DTMC with max. number of task retries per agent (i.e., largest possible model checked).\\
%\text{**} across all Pareto-front solutions.\\
%\textasciicircum{} EvoChecker returns 1. This is a float error as the same (non-parametrised DTMC) model tested in PRISM returns the depicted value.\\
OOM = out of memory. CS = retries set as in Table~\ref{table:vineyard_costs_prob}. All tasks in $\mathcal{M}_{1-2}$ are type $t3$. Model $\mathcal{M}_4$ is our vineyard case study.
\end{scriptsize}
\vspace{-5mm}
\end{table*}


% \begin{table}[]
% \caption{Model variants}
% \label{table:eval-modelsVariants}
% %\centering
% \sffamily
% \begin{scriptsize}
% \begin{center}
% \begin{tabular}{p{0.5cm}|llll}
% \toprule
% Model \\
% \midrule
% $\mathcal{M}_1$  \\
% $\mathcal{M}_2$ \\
% $\mathcal{M}_3$  \\
% $\mathcal{M}_4$  \\
% \bottomrule
% \end{tabular}
% \end{center}

% \end{scriptsize}
% \end{table}




% \begin{table*}[]
% \caption{Hybrid approach compared to a full-MDP model}
% %\url{https://docs.google.com/spreadsheets/d/1Iwyae02-TFwfa7iDuavsNNzRzTQacH21bkYkkwidn8A/edit?gid=1195719558#gid=1195719558}}
% \label{table:fullMDP}
% %\centering
% \sffamily
% \begin{scriptsize}
% \begin{center}
% \begin{tabular}{p{0.5cm}|p{1.0cm}lll|lllllp{0.5cm}}
% %\toprule
% \cline{2-11}
%  & \multicolumn{4}{c}{\textbf{Full MDP verification approach}} & \multicolumn{6}{c}{\textbf{Hybrid approach}} \\
% %\cline{2-11}
% \midrule
% Model & \multicolumn{1}{l}{\#states} & \multicolumn{1}{l}{\#trans} & \begin{tabular}[c]{@{}l@{}}max. prob \\ verif.\\ (time (s))\end{tabular} & \begin{tabular}[c]{@{}l@{}}min cost\\verif\\ (time (s))\end{tabular} & \# states* & \# trans* & max. prob** & min cost** & \begin{tabular}[c]{@{}l@{}}Heuristic\\ planner\\ time (s)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Verif. \&\\ search\\ time (m)\end{tabular} \\
% \midrule
% % problem1:
% % 2 tasks, 6 loc, 3 retries, 2 agents (1w, 1r)
% % problem2:
% % 3 tasks, 9 loc, 1 retry per task, 2 agents (1w, 1r)
% % problem3:
% % 3 tasks, 9 loc, n retries, 2 agents (1w, 1r)
% % problem4:
% % 10 tasks, 9 loc, n retries, 4 agents (2r 2w)

% %problem1 in data
% $\mathcal{M}_1$ & 54,011 & 219,732 & 0.99999 (0.14 s) & 4.06 (0.215 s) & 36 & 48 & 0.99994\textasciicircum{} & 5.06 & 0.71 & 2.13 \\ %p = 0.9999999999333901, 0.999946000729
% %problem2 in data
% $\mathcal{M}_2$ & 87,497 & 434,176 & 0.99910 (0.97 s) & 7.09~(1.48 s) & 14 & 17 & 0.97029 & 18.94 & 0.34 & 2.34 \\ % p= 0.999100269973, 0.9702989999999999
% %problem3 in data
% $\mathcal{M}_3$ & 270,100,547 & 1,351,524,022 & Timeout & Timeout & 398 & 553 & 0.99999 \textasciicircum{} & 19.15 & 0.33 & 12.41 \\ %0.99999999793485
% %problem4 in data
% $\mathcal{M}_4$ & OOM & OOM & - & - & 1,825,976 & 3,822,145 & 0.99999 & 38.18 & 2.23 & 13.47\\ %0.9999999963720143
% \bottomrule
% \end{tabular}
% \end{center}
% \text{*} from DTMC with max. number of task retries per agent (i.e., largest possible model)\\
% \text{**} across all Pareto-front solutions.\\
% \textasciicircum{} EvoChecker returns 1. This is a float error as the same (non-parametrised DTMC) model tested in PRISM returns 0.99999897669992.\\
% OOM = out of memory
% \end{scriptsize}
% \end{table*}






==> name.tex <==
\begin{lstlisting}[language=json,firstnumber=1,escapechar=!]
(define (problem robot_btrm-problem)
 (:domain robot_btrm-domain)
 (:objects !\colorbox{green!50}{l1 l2 l3 l4 l5 l6 l7 l8 l9}! - location)
 (:init 
	!\colorbox{green!50}{(path l1 l2) (path l2 l3) (path l4 l5)}!
	!\colorbox{green!50}{(path l5 l6) (path l7 l8) (path l8 l9)}!
	!\colorbox{green!50}{(path l2 l1) (path l3 l2) (path l5 l4)}!...
	!\colorbox{green!50}{(empty l2) (empty l3) (empty l4)...}!
	!\colorbox{green!50}{(task\_loc t1l4 l4) (task\_loc t1l6a l6)}!
	!\colorbox{green!50}{(task\_loc t1l6b l6) (task\_loc t1l7 l7)}!
	!\colorbox{green!50}{(task\_loc t2l5 l5) (task\_loc t2l8a l8)}!...
	!\colorbox{green!50}{(agent\_at worker1 l1) (agent\_at r1 l1)}!
	...
	!\colorbox{green!50}{($=$ (p\_success worker1 t1l4) 1)}!
	!\colorbox{green!50}{($=$ (p\_success worker1 t1l6a) 1)}!
	!\colorbox{green!50}{($=$ (p\_success worker1 t3l4) 0.99)}! 
        !\colorbox{green!50}{($=$ (p\_success worker1 t2l5) 0)}!...
)
(:goal
	!\colorbox{green!50}{(and (task\_done t1l4) (task\_done t1l6a)}!
	!\colorbox{green!50}{(task\_done t1l6b) (task\_done t1l7)}!...
)
 (:metric minimize (travel_dist))
)
\end{lstlisting}
